MMIST-ccRCC: A Real World Medical Dataset for the Development of Multi-Modal Systems

The acquisition of different data modalities can enhance our knowledge and understanding of various diseases, paving the way for a more personalized healthcare. Thus, medicine is progressively moving towards the generation of massive amounts of multi-modal data (\emph{e.g,} molecular, radiology, and histopathology). While this may seem like an ideal environment to capitalize data-centric machine learning approaches, most methods still focus on exploring a single or a pair of modalities due to a variety of reasons: i) lack of ready to use curated datasets; ii) difficulty in identifying the best multi-modal fusion strategy; and iii) missing modalities across patients. In this paper we introduce a real world multi-modal dataset called MMIST-CCRCC that comprises 2 radiology modalities (CT and MRI), histopathology, genomics, and clinical data from 618 patients with clear cell renal cell carcinoma (ccRCC). We provide single and multi-modal (early and late fusion) benchmarks in the task of 12-month survival prediction in the challenging scenario of one or more missing modalities for each patient, with missing rates that range from 26$\%$ for genomics data to more than 90$\%$ for MRI. We show that even with such severe missing rates the fusion of modalities leads to improvements in the survival forecasting. Additionally, incorporating a strategy to generate the latent representations of the missing modalities given the available ones further improves the performance, highlighting a potential complementarity across modalities. Our dataset and code are available here: https://multi-modal-ist.github.io/datasets/ccRCC

==> sec/4.1_table.tex <==
% Table 2
\begin{table}[t]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
Modality     & CT       & MRI & Pathology & AVG \\ \midrule 
%ACC & 0.9310      & 0.9333 & 0.5702    \\ 
%F1-Score & 0.6485     & 0.8800 & 0.5145      \\ \bottomrule
MIL Modalities  & 61.57      & 83.33  & 69.94  & - \\ \midrule 
Baselines       & 61.59      & 50.00  & 53.42  & 73.16  \\\midrule 
Late Fusion WS  & 65.00 & 73.33 & 73.16 & 73.16 & 73.15 \\
Late Fusion LW  & 73.85 & 61.66 & 69.36 & 69.36 & 69.35 \\\midrule 
Early Fusion Mean  & 88.18 & 73.33 & 83.23 & 83.23 & 82.32 \\
Early Fusion Cat  & 77.50 & 85.00 & 78.45 & 78.45 & 78.45 \\\midrule 
Early Fusion With Reconstruction Mean & 90.91 & 61.67 & 84.70 & 84.70 & 84.70 \\
Early Fusion With Reconstruction Cat & 85.45 & 56.67 & 83.27 & 83.27 & 83.27 \\ \bottomrule

\end{tabular}
\caption{Best Test BACC results for our experiments.}\label{tab:mil}
\end{table}


